Approximate Counting via Correlation Decay on Planar Graphs

We show for a broad class of counting problems, correlation decay (strong spatial mixing) implies FPTAS on planar graphs. The framework for the counting problems considered by us is the Holant problems with arbitrary constant-size domain and symmetric constraint functions. We define a notion of regularity on the constraint functions, which covers a wide range of natural and important counting problems, including all multi-state spin systems, counting graph homomorphisms, counting weighted matchings or perfect matchings, the subgraphs world problem transformed from the ferromagnetic Ising model, and all counting CSPs and Holant problems with symmetric constraint functions of constant arity. The core of our algorithm is a fixed-parameter tractable algorithm which computes the exact values of the Holant problems with regular constraint functions on graphs of bounded treewidth. By utilizing the locally tree-like property of apex-minor-free families of graphs, the parameterized exact algorithm implies an FPTAS for the Holant problem on these graph families whenever the Gibbs measure defined by the problem exhibits strong spatial mixing. We further extend the recursive coupling technique to Holant problems and establish strong spatial mixing for the ferromagnetic Potts model and the subgraphs world problem. As consequences, we have new deterministic approximation algorithms on planar graphs and all apex-minor-free graphs for several counting problems.

==> preamble.tex <==
\usepackage{amssymb, amsmath, amsthm}
\usepackage{mathrsfs}

%\theoremstyle{plain}
\newtheorem{thm}{Theorem}
\newtheorem{lem}[thm]{Lemma}
\newtheorem{prop}[thm]{Proposition}
\newtheorem{cor}[thm]{Corollary}
\newtheorem{fact}[thm]{Fact}


%\theoremstyle{definition}

\newtheorem{defn}[thm]{Definition}
\newtheorem{conj}[thm]{Conjecture}
\newtheorem{exmp}[thm]{Example}
%\newtheorem{claim}[thm]{Claim}

%\theoremstyle{remark}
\newtheorem{rem}[thm]{Remark}


\newcommand{\factorial}{\ensuremath{\mbox{\sc Factorial}}}

\newcommand{\ccr}[1]{{\color{red}#1}}
\newcommand{\ccb}[1]{{\color{blue}#1}}
\newcommand{\ccp}[1]{\underline{\color{purple}#1}}
\newcommand{\circo}[1]{\overset{\circ}{#1}}
\newcommand{\mb}{\mathbb}
\newcommand{\mc}{\mathcal}
\newcommand{\ms}{\mathscr}


\newcommand{\IFP}{\mathsf{IFP}}
\newcommand{\ifp}{\mathsf{ifp}}
\newcommand{\FO}{\mathsf{FO}}
\newcommand{\MSO}{\mathsf{MSO}}





\newcommand{\FPT}{\mathbf{FPT}}
\newcommand{\EXPT}{\mathbf{EXPT}}
\newcommand{\EPT}{\mathbf{EPT}}
\newcommand{\SUBEPT}{\mathbf{SUBEPT}}
\renewcommand{\P}{\mathbf{PTIME}}
\newcommand{\NP}{\mathbf{NP}}
\newcommand{\coNP}{\mathbf{coNP}}
\newcommand{\PSPACE}{\mathbf{PSPACE}}
\newcommand{\XP}{\mathbf{XP}}
\newcommand{\paraNP}{\mathbf{para}\mbox{-}\NP}
\newcommand{\WP}{\mathbf{W[P]}}
\newcommand{\Wt}{\mathbf{W[t]}}
\newcommand{\At}{\mathbf{A[t]}}
\newcommand{\Wone}{\mathbf{W[1]}}
\newcommand{\Aone}{\mathbf{A[1]}}
\newcommand{\AWstar}{\mathbf{AW[*]}}
\newcommand{\EXP}{\mathbf{EXPTIME}}
\newcommand{\DTIME}{\mathbf{DTIME}}
\newcommand{\NTIME}{\mathbf{NTIME}}
\renewcommand{\L}{\mathbf{L}}
\newcommand{\NL}{\mathbf{NL}}
\newcommand{\SPACE}{\mathbf{SPACE}}
\newcommand{\NSPACE}{\mathbf{NSPACE}}
\newcommand{\TIME}{\mathbf{TIME}}
\newcommand{\NEXP}{\mathbf{NEXP}}
\newcommand{\PH}{\mathbf{PH}}



\newcommand{\PROP}{\mathsf{PROP}}
\newcommand{\CIRC}{\mathsf{CIRC}}
\newcommand{\CNF}{\mathsf{CNF}}
\newcommand{\DNF}{\mathsf{DNF}}
\newcommand{\lGamma}{\mathsf{\Gamma}}
\newcommand{\lDelta}{\mathsf{\Delta}}
\newcommand{\lSigma}{\mathsf{\Sigma}}
\newcommand{\lPi}{\mathsf{\Pi}}
\newcommand{\alphSig}{\mathsf{\Sigma}}


\newcommand{\natN}{\mathbb{N}}

\newcommand{\fptequiv}{\equiv^{\mathrm{fpt}}}
\newcommand{\fptle}{\le^{\mathrm{fpt}}}
\newcommand{\fptl}{<^{\mathrm{fpt}}}
\newcommand{\eptequiv}{\equiv^{\mathrm{ept}}}
\newcommand{\eptle}{\le^{\mathrm{ept}}}
\newcommand{\eptl}{<^{\mathrm{ept}}}




\newcommand{\sideremark}[1]{\marginpar{\raggedright\footnotesize #1}}

\newlength{\probwidth}
\setlength{\probwidth}{3cm}

\newcommand{\prob}[3][8]{
\begin{center}
\normalfont \fbox{
\begin{tabular}[t]{rp{#1cm}}\textit{Input:}&#2.\\\textit{Problem:}&#3
\end{tabular}}
\end{center}}

\newcommand{\pprob}[4][8]{
\begin{center}
\normalfont\fbox{
\begin{tabular}[t]{rp{#1cm}}\textit{Input:}&#2.\\\textit{Parameter:}&#3.\\\textit{Problem:}&#4
\end{tabular}}
\end{center}}

\newcommand{\nprob}[4][8]{
\begin{center}\normalfont\fbox{
\addtolength{\probwidth}{#1cm}\parbox{\probwidth}{\textsc{#2}\\\hspace*{1.5em}
\begin{tabular}[t]{rp{#1cm}}%\textsc{#2} \
\textit{Input:}&#3.\\\textit{Problem:}&#4
\end{tabular}}}
\end{center}}

\newcommand{\npprob}[5][8]{
\begin{center}\normalfont\fbox{
\addtolength{\probwidth}{#1cm}\parbox{\probwidth}{\textsc{#2}\\\hspace*{1.5em}
\begin{tabular}[t]{rp{#1cm}}%\textsc{#2} \
\textit{Input:}&#3.\\\textit{Parameter:}&#4.\\\textit{Problem:}&#5
\end{tabular}}}
\end{center}}

\newcommand{\nppprob}[5][8]{
\begin{center}
\normalfont\fbox{\addtolength{\probwidth}{#1cm}
\parbox{\probwidth}{\textsc{#2}\\\hspace*{1.5em}
\begin{tabular}[t]{rp{#1cm}}
\textit{Input:}&#3.\\\textit{Parameter:}&#4.\\\textit{Problem:}&#5
\end{tabular}}}
\end{center}}


\newcommand{\noptprob}[6][8]{
\begin{center}\normalfont\fbox{
\addtolength{\probwidth}{#1cm}\parbox{\probwidth}{\textsc{#2}\\\hspace*{1.5em}
\begin{tabular}[t]{rp{#1cm}}%\textsc{#2} \
\textit{Input:}&#3.\\\textit{Solution:}&#4.\\
\textit{Cost:}&#5.\\\textit{Goal:}&#6.
\end{tabular}}}
\end{center}}


\newcommand{\algo}[5][9]{
  \begin{center}\normalfont
    \fbox{
      \addtolength{\probwidth}{#1cm}
      \parbox{\probwidth} {
        #2\\

        \smallskip
        \begin{tabular}[t]{lp{#1cm}}
          \textbf{Input:}&#3.\\
          \textbf{Output:}&#4.
        \end{tabular}\\
        #5
        }
      }
  \end{center}
}

